PoseMamba: Monocular 3D Human Pose Estimation with Bidirectional Global-Local Spatio-Temporal State Space Model

Transformers have significantly advanced the field of 3D human pose estimation (HPE). However, existing transformer-based methods primarily use self-attention mechanisms for spatio-temporal modeling, leading to a quadratic complexity, unidirectional modeling of spatio-temporal relationships, and insufficient learning of spatial-temporal correlations. Recently, the Mamba architecture, utilizing the state space model (SSM), has exhibited superior long-range modeling capabilities in a variety of vision tasks with linear complexity. In this paper, we propose PoseMamba, a novel purely SSM-based approach with linear complexity for 3D human pose estimation in monocular video. Specifically, we propose a bidirectional global-local spatio-temporal SSM block that comprehensively models human joint relations within individual frames as well as temporal correlations across frames. Within this bidirectional global-local spatio-temporal SSM block, we introduce a reordering strategy to enhance the local modeling capability of the SSM. This strategy provides a more logical geometric scanning order and integrates it with the global SSM, resulting in a combined global-local spatial scan. We have quantitatively and qualitatively evaluated our approach using two benchmark datasets: Human3.6M and MPI-INF-3DHP. Extensive experiments demonstrate that PoseMamba achieves state-of-the-art performance on both datasets while maintaining a smaller model size and reducing computational costs. The code and models will be released.

==> sup_files/checklist.tex <==
\section{Reproducibility Checklist}
\paragraph{This paper:}
\begin{itemize}
    \item  Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) {\bf yes}
  \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) {\bf yes}
    
   \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no)  {\bf yes}
    
\end{itemize}

\paragraph{Does this paper make theoretical contributions? (yes/no) {\bf no}}
\paragraph{If yes, please complete the list below.}
\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
\item Proofs of all novel claims are included. (yes/partial/no)
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\paragraph{Does this paper rely on one or more datasets? (yes/no) {\bf yes}}
\paragraph{If yes, please complete the list below.}
\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) {\bf yes}
\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) {\bf NA}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) {\bf NA}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) {\bf yes}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) {\bf yes}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) {\bf NA}
\end{itemize}

\paragraph{Does this paper include computational experiments? (yes/no) {\bf yes}}
\paragraph{If yes, please complete the list below.}
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (yes/partial/no) {\bf no}
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) {\bf no}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) 
 {\bf yes}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) {\bf no}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) {\bf yes}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) {\bf yes}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) {\bf yes}
\item This paper states the number of algorithm runs used to compute each reported result. (yes/no) {\bf yes}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) {\bf yes}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) {\bf no}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) {\bf yes}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) {\bf yes}
\end{itemize}





